Singing Voice Conversion with Disentangled Representations of Singer and Vocal Technique Using Variational Autoencoders

We propose a flexible framework that deals with both singer conversion and singers vocal technique conversion. The proposed model is trained on non-parallel corpora, accommodates many-to-many conversion, and leverages recent advances of variational autoencoders. It employs separate encoders to learn disentangled latent representations of singer identity and vocal technique separately, with a joint decoder for reconstruction. Conversion is carried out by simple vector arithmetic in the learned latent spaces. Both a quantitative analysis as well as a visualization of the converted spectrograms show that our model is able to disentangle singer identity and vocal technique and successfully perform conversion of these attributes. To the best of our knowledge, this is the first work to jointly tackle conversion of singer identity and vocal technique based on a deep learning approach.

==> full-ref.tex <==
% ICLR 2019
@inproceedings{DBLP:conf/iclr/HsuZWZWWCJCSNP19,
  author    = {Wei{-}Ning Hsu and
               Yu Zhang and
               Ron J. Weiss and
               Heiga Zen and
               Yonghui Wu and
               Yuxuan Wang and
               Yuan Cao and
               Ye Jia and
               Zhifeng Chen and
               Jonathan Shen and
               Patrick Nguyen and
               Ruoming Pang},
  title     = {Hierarchical Generative Modeling for Controllable Speech Synthesis},
  booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  year      = {2019},
  crossref  = {DBLP:conf/iclr/2019},
  url       = {https://openreview.net/forum?id=rygkk305YQ},
  timestamp = {Thu, 25 Jul 2019 14:25:40 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/HsuZWZWWCJCSNP19},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/iclr/2019,
  title     = {7th International Conference on Learning Representations, {ICLR} 2019,
               New Orleans, LA, USA, May 6-9, 2019},
  publisher = {OpenReview.net},
  year      = {2019},
  url       = {https://openreview.net/group?id=ICLR.cc/2019/Conference},
  timestamp = {Thu, 25 Jul 2019 13:03:15 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/2019},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

% ================== ISMIR 2018 ================== 
@inproceedings{DBLP:conf/ismir/WilkinsSWP18,
  author    = {Julia Wilkins and
               Prem Seetharaman and
               Alison Wahl and
               Bryan Pardo},
  title     = {VocalSet: {A} Singing Voice Dataset},
  booktitle = {Proceedings of the 19th International Society for Music Information
               Retrieval Conference, {ISMIR} 2018, Paris, France, September 23-27,
               2018},
  pages     = {468--474},
  year      = {2018},
  crossref  = {DBLP:conf/ismir/2018},
  url       = {http://ismir2018.ircam.fr/doc/pdfs/114\_Paper.pdf},
  timestamp = {Tue, 20 Nov 2018 15:33:12 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/ismir/WilkinsSWP18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/ismir/2018,
  editor    = {Emilia G{\'{o}}mez and
               Xiao Hu and
               Eric Humphrey and
               Emmanouil Benetos},
  title     = {Proceedings of the 19th International Society for Music Information
               Retrieval Conference, {ISMIR} 2018, Paris, France, September 23-27,
               2018},
  year      = {2018},
  isbn      = {978-2-9540351-2-3},
  timestamp = {Tue, 20 Nov 2018 15:32:44 +0100},
  biburl    = {https://dblp.org/rec/bib/conf/ismir/2018},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

% ICLR 2015
@inproceedings{DBLP:journals/corr/KingmaB14,
  author    = {Diederik P. Kingma and
               Jimmy Ba},
  title     = {Adam: {A} Method for Stochastic Optimization},
  booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  crossref  = {DBLP:conf/iclr/2015},
  url       = {http://arxiv.org/abs/1412.6980},
  timestamp = {Thu, 25 Jul 2019 14:25:37 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/KingmaB14},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/iclr/2015,
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {3rd International Conference on Learning Representations, {ICLR} 2015,
               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
  year      = {2015},
  url       = {https://iclr.cc/archive/www/doku.php\%3Fid=iclr2015:accepted-main.html},
  timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/2015},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


% ICLR 2014
@inproceedings{DBLP:journals/corr/KingmaW13,
  author    = {Diederik P. Kingma and
               Max Welling},
  title     = {Auto-Encoding Variational Bayes},
  booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
               Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year      = {2014},
  crossref  = {DBLP:conf/iclr/2014},
  url       = {http://arxiv.org/abs/1312.6114},
  timestamp = {Thu, 04 Apr 2019 13:20:07 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/KingmaW13},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/iclr/2014,
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {2nd International Conference on Learning Representations, {ICLR} 2014,
               Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year      = {2014},
  url       = {https://openreview.net/group?id=ICLR.cc/2014},
  timestamp = {Thu, 04 Apr 2019 13:20:07 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/iclr/2014},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


% AISTATS 2010
@inproceedings{DBLP:journals/jmlr/GlorotB10,
  author    = {Xavier Glorot and
      Yoshua Bengio},
  title     = {Understanding the difficulty of training deep feedforward neural networks},
  booktitle = {Proceedings of the Thirteenth International Conference on Artificial
      Intelligence and Statistics, {AISTATS} 2010, Chia Laguna Resort, Sardinia,
      Italy, May 13-15, 2010},
  pages     = {249--256},
  year      = {2010},
  crossref  = {DBLP:conf/aistats/2010},
  url       = {http://proceedings.mlr.press/v9/glorot10a.html},
  timestamp = {Wed, 29 May 2019 08:41:47 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/jmlr/GlorotB10},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@proceedings{DBLP:conf/aistats/2010,
  editor    = {Yee Whye Teh and
      D. Mike Titterington},
  title     = {Proceedings of the Thirteenth International Conference on Artificial
      Intelligence and Statistics, {AISTATS} 2010, Chia Laguna Resort, Sardinia,
      Italy, May 13-15, 2010},
  series    = {{JMLR} Proceedings},
  volume    = {9},
  publisher = {JMLR.org},
  year      = {2010},
  url       = {http://proceedings.mlr.press/v9/},
  timestamp = {Wed, 29 May 2019 08:41:44 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/aistats/2010},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

% attention
@inproceedings{sonderby2015convolutional,
  title={Convolutional LSTM networks for subcellular localization of proteins},
  author={S{\o}nderby, S{\o}ren Kaae and S{\o}nderby, Casper Kaae and Nielsen, Henrik and Winther, Ole},
  booktitle={International Conference on Algorithms for Computational Biology},
  pages={68--80},
  year={2015},
  organization={Springer}
}

@inproceedings{collin2015feedforward,
  author    = {C. Raffel and D. P. Ellis},
  title     = {Feed-forward networks with attention can solve some long-term memory problems},
  booktitle = {International Conference on Learning Representations, {ICLR} 2016,
  workshop track},
  year      = {2016},
}

% disentanglement
@inproceedings{hsu2019hierarchical,
  author    = {W.-N. Hsu and Y. Zhang, R. J. Weiss and H. Zen and Y. Wu and Y. Wang and Y. Cao and Y. Jia and Z. Chen and J. Shen and P. Nguyen and R. Pang},
  title     = {Hierarchical Generative Modeling for Controllable Speech Synthesis},
  booktitle = {International Conference on Learning Representations, {ICLR} 2019},
  year      = {2019},
}

@inproceedings{luo2019disentangle,
  author    = {Y.-J. Luo and K. Agres and D. Herremans},
  title     = {Learning Disentangled Representations of Timbre and Pitch for Musical Instrument Sounds Using Gaussian Mixture Variational Autoencoders},
  booktitle = {Proceedings of the 19th International Society for Music Information
               Retrieval Conference, {ISMIR} 2019},
  year      = {2019},
}

%VC
@article{lorenzo2018voice,
  title={The voice conversion challenge 2018: Promoting development of parallel and nonparallel methods},
  author={Lorenzo-Trueba, Jaime and Yamagishi, Junichi and Toda, Tomoki and Saito, Daisuke and Villavicencio, Fernando and Kinnunen, Tomi and Ling, Zhenhua},
  journal={arXiv preprint arXiv:1804.04262},
  year={2018}
}

@inproceedings{sun2015voice,
  title={Voice conversion using deep bidirectional long short-term memory based recurrent neural networks},
  author={Sun, Lifa and Kang, Shiyin and Li, Kun and Meng, Helen},
  booktitle={2015 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={4869--4873},
  year={2015},
  organization={IEEE}
}

@INPROCEEDINGS{sun2015dblstm,
author={L. {Sun} and S. {Kang} and K. {Li} and H. {Meng}},
booktitle={2015 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
title={Voice conversion using deep Bidirectional Long Short-Term Memory based Recurrent Neural Networks},
year={2015},
volume={},
number={},
pages={4869-4873},
keywords={recurrent neural nets;speech processing;voice conversion;deep bidirectional long short-term memory based recurrent neural networks;DBLSTM-RNNs;temporal correlations;DNNs;frame-based methods;speech frames;sequence-based conversion method;long-range context-dependency;acoustic trajectory;mean opinion scores;Speech;Training;Recurrent neural networks;Logic gates;Context;Acoustics;voice conversion;bidirectional long short-term memory;recurrent neural networks;dynamic features},
doi={10.1109/ICASSP.2015.7178896},
ISSN={},
month={April},}

%SVC
@inproceedings{villavicencio2010applying,
  title={Applying voice conversion to concatenative singing-voice synthesis},
  author={Villavicencio, Fernando and Bonada, Jordi},
  booktitle={Eleventh Annual Conference of the International Speech Communication Association},
  year={2010}
}


@INPROCEEDINGS{doi2012singingvoicconversion,
author={H. {Doi} and T. {Toda} and T. {Nakano} and M. {Goto} and S. {Nakamura}},
booktitle={Proceedings of The 2012 Asia Pacific Signal and Information Processing Association Annual Summit and Conference},
title={Singing voice conversion method based on many-to-many eigenvoice conversion and training data generation using a singing-to-singing synthesis system},
year={2012},
volume={},
number={},
pages={1-6},
keywords={eigenvalues and eigenfunctions;speech processing;training data generation;voice quality;voice identity;signal-processing technology;singing voice conversion method;many-to-many eigenvoice conversion;EVC;arbitrary source singer;arbitrary target singer;voice conversion model;singing-to-singing synthesis system;VocaListener;parallel data;Training;Vectors;Training data;Acoustics;Data models;Adaptation models;Accuracy},
doi={},
ISSN={},
month={Dec},}

@inproceedings{kobayashi2014statistical,
  title={Statistical singing voice conversion with direct waveform modification based on the spectrum differential},
  author={Kobayashi, Kazuhiro and Toda, Tomoki and Neubig, Graham and Sakti, Sakriani and Nakamura, Satoshi},
  booktitle={Fifteenth Annual Conference of the International Speech Communication Association},
  year={2014}
}

@inproceedings{sisman2019singan,
author = {Sisman, Berrak and Vijayan, Karthika and Dong, Minghui and Li, Haizhou},
year = {2019},
month = {09},
pages = {},
title = {SINGAN: Singing Voice Conversion with Generative Adversarial Networks}
}







% non-parrallel SVC and VC
@INPROCEEDINGS{Hsu2016vae, 
author={C.-C. Hsu and H.-T. Hwang and Y.-C. Wu and Y. Tsao and H.-M. Wang}, 
booktitle={2016 Asia-Pacific Signal and Information Processing Association Annual Summit and Conference (APSIPA)}, 
title={Voice conversion from non-parallel corpora using variational auto-encoder}, 
year={2016}, 
volume={}, 
number={}, 
pages={1-6}, 
}


@INPROCEEDINGS{Kameoka2018StarGAN, 
author={H. {Kameoka} and T. {Kaneko} and K. {Tanaka} and N. {Hojo}}, 
booktitle={2018 IEEE Spoken Language Technology Workshop (SLT)}, 
title={StarGAN-VC: non-parallel many-to-many Voice Conversion Using Star Generative Adversarial Networks}, 
year={2018}, 
volume={}, 
number={}, 
pages={266-273}, 
keywords={learning (artificial intelligence);speaker recognition;StarGAN-VC;voice conversion;star generative adversarial networks;speech generator training;different attribute domains;single generator network;converted speech signals;real-time implementations;speaker identity conversion task;state-of-the-art method;nonparallel many-to-many voice conversion;many-to-many mappings;realistic sounding speech;speaker identity conversion;variational autoencoding GAN;Training;Acoustics;Gallium nitride;Generators;Decoding;Speech recognition;Task analysis;Voice conversion (VC);non-parallel VC;many-to-many VC;generative adversarial networks (GANs);CycleGAN-VC;StarGAN-VC}, 
doi={10.1109/SLT.2018.8639535}, 
ISSN={}, 
month={Dec},}


@misc{zhang2019nonparallel,
    title={Non-Parallel Sequence-to-Sequence Voice Conversion with Disentangled Linguistic and Speaker Representations},
    author={Jing-Xuan Zhang and Zhen-Hua Ling and Li-Rong Dai},
    year={2019},
    eprint={1906.10508},
    archivePrefix={arXiv},
    primaryClass={eess.AS}
}

@inproceedings{DBLP:conf/interspeech/ChouYLL18,
  author    = {Ju{-}Chieh Chou and
               Cheng{-}chieh Yeh and
               Hung{-}yi Lee and
               Lin{-}Shan Lee},
  title     = {Multi-target Voice Conversion without Parallel Data by Adversarially
               Learning Disentangled Audio Representations},
  booktitle = {Interspeech 2018, 19th Annual Conference of the International Speech
               Communication Association, Hyderabad, India, 2-6 September 2018.},
  pages     = {501--505},
  year      = {2018},
  crossref  = {DBLP:conf/interspeech/2018},
  url       = {https://doi.org/10.21437/Interspeech.2018-1830},
  doi       = {10.21437/Interspeech.2018-1830},
  timestamp = {Mon, 15 Jul 2019 08:28:46 +0200},
  biburl    = {https://dblp.org/rec/bib/conf/interspeech/ChouYLL18},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{chen2019singing,
  title={Singing voice conversion with non-parallel data},
  author={Chen, Xin and Chu, Wei and Guo, Jinxi and Xu, Ning},
  booktitle={2019 IEEE Conference on Multimedia Information Processing and Retrieval (MIPR)},
  pages={292--296},
  year={2019},
  organization={IEEE}
}

@article{nachmani2019unsupervised,
  title={Unsupervised Singing Voice Conversion},
  author={Nachmani, Eliya and Wolf, Lior},
  journal={arXiv preprint arXiv:1904.06590},
  year={2019}
}

%GMVAE
@article{dilokthanakul2016deep,
  title={Deep unsupervised clustering with gaussian mixture variational autoencoders},
  author={N. Dilokthanakul and P. A. M. Mediano and M. Garnelo and M. C.-H. Lee and H. Salimbeni and K. Arulkumaran and M. Shanahan},
  journal={arXiv preprint arXiv:1611.02648},
  year={2016}
}

@inproceedings{kingma2014semi,
  title={Semi-supervised learning with deep generative models},
  author={D. P. Kingma and S. Mohamed and D. J. Rezende and M. Welling},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3581--3589},
  year={2014}
}

@inproceedings{jiang2016variational,
  title={Variational deep embedding: An unsupervised and generative approach to clustering},
  author={Z. Jiang and Y. Zheng and H. Tan and B. Tang and H. Zhou},
  booktitle={International Joint Conference on Artificial Intelligence},
  year={2017}
}


@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  booktitle={Advances in neural information processing systems},
  pages={2672--2680},
  year={2014}
}

@article{ganin2016domain,
  title={Domain-adversarial training of neural networks},
  author={Ganin, Yaroslav and Ustinova, Evgeniya and Ajakan, Hana and Germain, Pascal and Larochelle, Hugo and Laviolette, Fran{\c{c}}ois and Marchand, Mario and Lempitsky, Victor},
  journal={The Journal of Machine Learning Research},
  volume={17},
  number={1},
  pages={2096--2030},
  year={2016},
  publisher={JMLR. org}
}


